Fight or Flight: Cosmic Ray-Induced Phonons and the Quantum Surface Code

Recent work has identified cosmic ray events as an error source limiting the lifetime of quantum data. These errors are correlated and affect a large number of qubits, leading to the loss of data across a quantum chip. Previous works attempting to address the problem in hardware or by building distributed systems still have limitations. We approach the problem from a different perspective, developing a new hybrid hardware-software-based strategy based on the 2-D surface code, assuming the parallel development of a hardware strategy that limits the phonon propagation radius. We propose to flee the area: move the logical qubits far enough away from the strike's epicenter to maintain our logical information. Specifically, we: (1) establish the minimum hardware requirements needed for our approach; (2) propose a mapping for moving logical qubits; and (3) evaluate the possible choice of the code distance. Our analysis considers two possible cosmic ray events: those far from both ``holes'' in the surface code and those near or overlapping a hole. We show that the probability that the logical qubit will be destroyed can be reduced from 100% to the range 4% to 15% depending on the time required to move the logical qubit.

==> custom-command.tex <==
% ================== CUSTOM COMMANDS ==================
% for adding notes to self
\usepackage[svgnames, table]{xcolor}
\usepackage{tabularx, makecell, linegoal}
% \usepackage{todonotes}

\newcommand{\mynote}[1]{\medskip\par\textbf{\small Note}\quad\setlength{\extrarowheight}{2pt}\begin{tabularx}{\linegoal}{X}
\Xhline{1pt}
\rowcolor{WhiteSmoke!80!Lavender}#1 \\
\Xhline{1pt}
\end{tabularx}}
\usepackage{ifthen}

\newboolean{ShowComments}
\setboolean{ShowComments}{true}  % change to true to show remaining colorful author comments. 
                                 % change to false to hide all author comments.
\ifthenelse{\boolean{ShowComments}}%
	{
		\newcommand{\ColorComment}[3]{%
				{\colorbox{#1}{\color{White}   \textsf{\textbf{#2}}} \textcolor{#1}{#3}}}%  Colorful box, initials, phrase 
        \newcommand{\TR}[1]{\textcolor{Red}{#1}}
        \newcommand{\TB}[1]{\textcolor{Red}{#1}}
        \newcommand{\TO}[1]{\textcolor{Red}{#1}}
	}%
	{
		\newcommand{\ColorComment}[3]{}%  Do nothing at all
        \newcommand{\TR}[1]{#1}
        \newcommand{\TB}[1]{#1}
        \newcommand{\TO}[1]{#1}
	}%

% new commands
%\newcommand{\TR}{\textcolor{red}}
%\newcommand{\TB}{\textcolor{blue}}
%\renewcommand\TR[1]{}
%\renewcommand\TB[1]{}
\definecolor{rdvcolor}{rgb}{0,0.5,0}\newcommand{\rdv}[1]{\ColorComment{rdvcolor}{rdv}{#1}}
\definecolor{satohcolor}{RGB}{254,125,106}\newcommand{\satoh}[1]{\ColorComment{satohcolor}{satoh}{#1}}
\definecolor{michalcolor}{RGB}{255,127,80}\newcommand{\michal}[1]{\ColorComment{michalcolor}{michal}{#1}}
\definecolor{naphanncolor}{RGB}{112, 51, 173}\newcommand{\naphann}[1]{\ColorComment{naphanncolor}{whit3z}{#1}}

%% This part goes in preamble
\newcommand{\dummyfig}[1]{
  \centering
  \fbox{
    \begin{minipage}[c][0.33\textheight][c]{0.45\textwidth}
      \centering{#1}
    \end{minipage}
  }
}
\newcommand*\mean[1]{\overline{#1}}

% ============ custom command ==============
